Entropy-dissipation Informed Neural Network for McKean-Vlasov Type PDEs

We extend the concept of self-consistency for the Fokker-Planck equation (FPE) to the more general McKean-Vlasov equation (MVE). While FPE describes the macroscopic behavior of particles under drift and diffusion, MVE accounts for the additional inter-particle interactions, which are often highly singular in physical systems. Two important examples considered in this paper are the MVE with Coulomb interactions and the vorticity formulation of the 2D Navier-Stokes equation. We show that a generalized self-consistency potential controls the KL-divergence between a hypothesis solution to the ground truth, through entropy dissipation. Built on this result, we propose to solve the MVEs by minimizing this potential function, while utilizing the neural networks for function approximation. We validate the empirical performance of our approach by comparing with state-of-the-art NN-based PDE solvers on several example problems.

==> math_command_information.tex <==
\section{Default Notation}

In an attempt to encourage standardized notation, we have included the
notation file from the textbook, \textit{Deep Learning}
\cite{goodfellow2016deep} available at
\url{https://github.com/goodfeli/dlbook_notation/}.  Use of this style
is not required and can be disabled by commenting out
\texttt{math\_commands.tex}.


\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
	$\displaystyle a$ & A scalar (integer or real)\\
	$\displaystyle \va$ & A vector\\
	$\displaystyle \mA$ & A matrix\\
	$\displaystyle \tA$ & A tensor\\
	$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
	$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
	$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
	$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
	$\displaystyle \ra$ & A scalar random variable\\
	$\displaystyle \rva$ & A vector-valued random variable\\
	$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
	$\displaystyle \sA$ & A set\\
	$\displaystyle \R$ & The set of real numbers \\
	$\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
	$\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
	$\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
	$\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
	$\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
	$\displaystyle \gG$ & A graph\\
	$\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\vspace{0.25cm}


\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
	$\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
	$\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
	$\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
	$\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
	$\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
	$\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
	$\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
	$\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup
\vspace{0.25cm}


\centerline{\bf Calculus}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
	% NOTE: the [2ex] on the next line adds extra height to that row of the table.
	% Without that command, the fraction on the first line is too tall and collides
	% with the fraction on the second line.
	$\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
	$\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
	$\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
	$\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
	$\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
	$\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
	$\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
	$\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
	$\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
	$\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
	$\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
	a variable whose type has not been specified\\
	$\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
	$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
	$\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
	$\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
	$\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
	$\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
	$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
	over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
	$\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
	$\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
	$\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
	(Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
	$\displaystyle \log x$ & Natural logarithm of $x$ \\
	$\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
	$\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
	$\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
	$\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
	$\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
	$\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
\end{tabular}
\egroup
\vspace{0.25cm}



%\section{Final instructions}
%Do not change any aspects of the formatting parameters in the style files.
%In particular, do not modify the width or length of the rectangle the text
%should fit into, and do not change font sizes (except perhaps in the
%\textsc{References} section; see below). Please note that pages should be
%numbered.
%
%\section{Preparing PostScript or PDF files}
%
%Please prepare PostScript or PDF files with paper size ``US Letter'', and
%not, for example, ``A4''. The -t
%letter option on dvips will produce US Letter files.
%
%Consider directly generating PDF files using \verb+pdflatex+
%(especially if you are a MiKTeX user).
%PDF figures must be substituted for EPS figures, however.
%
%Otherwise, please generate your PostScript and PDF files with the following commands:
%\begin{verbatim}
%	dvips mypaper.dvi -t letter -Ppdf -G0 -o mypaper.ps
%	ps2pdf mypaper.ps mypaper.pdf
%\end{verbatim}
%
%\subsection{Margins in LaTeX}
%
%Most of the margin problems come from figures positioned by hand using
%\verb+\special+ or other commands. We suggest using the command
%\verb+\includegraphics+
%from the graphicx package. Always specify the figure width as a multiple of
%the line width as in the example below using .eps graphics
%\begin{verbatim}
%	\usepackage[dvips]{graphicx} ...
%	\includegraphics[width=0.8\linewidth]{myfile.eps}
%\end{verbatim}
%or % Apr 2009 addition
%\begin{verbatim}
%	\usepackage[pdftex]{graphicx} ...
%	\includegraphics[width=0.8\linewidth]{myfile.pdf}
%\end{verbatim}
%for .pdf graphics.
%See section~4.4 in the graphics bundle documentation (\url{http://www.ctan.org/tex-archive/macros/latex/required/graphics/grfguide.ps})
%
%A number of width problems arise when LaTeX cannot properly hyphenate a
%line. Please give LaTeX hyphenation hints using the \verb+\-+ command.
%
%\subsubsection*{Author Contributions}
%If you'd like to, you may include  a section for author contributions as is done
%in many journals. This is optional and at the discretion of the authors.
%
%\subsubsection*{Acknowledgments}
%Use unnumbered third level headings for the acknowledgments. All
%acknowledgments, including those to funding agencies, go at the end of the paper.

